Multi-Resolution Hashing for Fast Pairwise Summations

A basic computational primitive in the analysis of massive datasets is summing simple functions over a large number of objects. Modern applications pose an additional challenge in that such functions often depend on a parameter vector $y$ (query) that is unknown a priori. Given a set of points $X\subset \mathbb{R}^{d}$ and a pairwise function $w:\mathbb{R}^{d}\times \mathbb{R}^{d}\to [0,1]$, we study the problem of designing a data-structure that enables sublinear-time approximation of the summation $Z_{w}(y)=\frac{1}{|X|}\sum_{x\in X}w(x,y)$ for any query $y\in \mathbb{R}^{d}$. By combining ideas from Harmonic Analysis (partitions of unity and approximation theory) with Hashing-Based-Estimators [Charikar, Siminelakis FOCS'17], we provide a general framework for designing such data structures through hashing that reaches far beyond what previous techniques allowed. A key design principle is a collection of $T\geq 1$ hashing schemes with collision probabilities $p_{1},\ldots, p_{T}$ such that $\sup_{t\in [T]}\{p_{t}(x,y)\} = \Theta(\sqrt{w(x,y)})$. This leads to a data-structure that approximates $Z_{w}(y)$ using a sub-linear number of samples from each hash family. Using this new framework along with Distance Sensitive Hashing [Aumuller, Christiani, Pagh, Silvestri PODS'18], we show that such a collection can be constructed and evaluated efficiently for any log-convex function $w(x,y)=e^{\phi(\langle x,y\rangle)}$ of the inner product on the unit sphere $x,y\in \mathcal{S}^{d-1}$. Our method leads to data structures with sub-linear query time that significantly improve upon random sampling and can be used for Kernel Density or Partition Function Estimation. We provide extensions of our result from the sphere to $\mathbb{R}^{d}$ and from scalar functions to vector functions.

==> hashing.tex <==
\subsection{Distance Sensitive Hashing on the Sphere}\label{sec:hashing}
In this section, we describe the hashing scheme of \cite{aumuller2017distance} and give slightly different bounds on the collision probability utilizing results from \cite{szarek1999nonsymmetric,hashorva2003multivariate} for Gaussian integrals.
\subsection{Locality Sensitive Hashing on the unit Sphere}
We define the hash family $\mathcal{D}_{+}=\mathcal{D}_{+}(t,\zeta)$ that takes as parameters real numbers $t>0$, $\zeta\in(0,1)$ and defines a pair of hash functions $h_{+}:\mathcal{S}^{d-1}\to  [m]\cup \{m+1\}$ and $g_{+}:\mathcal{S}^{d-1}\to [m]\cup\{m+2\}$, where $m$ is given by
\begin{equation}
m(t,\zeta )= \left\lceil \sqrt{2\pi}(t+1)\log(\frac{2}{\zeta}) e^{\frac{t^{2}}{2}}\right\rceil  
\end{equation}
To define the functions $h_{+},g_{+}$, we sample $m$ normal random vectors $g_{1},\ldots, g_{m}\stackrel{i.i.d.}{\sim}\mathcal{N}(0, I_{d})$ and use them to create $m+2$ hash buckets through the mappings
\begin{align}
h_{+}(x) &:= \min\left( \{i\bigr|\langle x, g_{i}\rangle\geq t \}\cup \{m+1\}\right)\\
g_{+}(x) &:= \min \left( \{i\bigr|\langle x, g_{i}\rangle\geq t \}\cup \{m+2\}\right)
\end{align}
The time and memory required for evaluating the function are both bounded by $O(dm)=O(dt \log(\frac{1}{\zeta})e^{\frac{t^{2}}{2}})$. We also define the hash family $\mathcal{D}_{-}(t,\zeta)$ that is identical to $\mathcal{D}_{+}$ except from that fact that  instead of using $g_{+}$ we use:
\begin{equation}
g_{-}(x) := \min \left( \{i\bigr|\langle x, g_{i}\rangle\geq -t \}\cup \{m+2\}\right)
\end{equation}
The need to use a pair of hash functions arises from the fact that we treat the points in the dataset $X$ and the queries differently. We will write $(h,g)\sim \mathcal{D}_{\pm}$ to indicate such pairs of hash functions. Due to isotropy of the normal distribution the collision probability is only a function of $\langle x,y\rangle$,
\begin{equation}
\P_{(h,g)\sim D_{\pm}}[h(y)=g(x)] = p_{\pm}(\langle x, y\rangle)
\end{equation}
and satisfies $p_{+}(\rho)=p_{-}(-\rho)$ for all $\rho\in[-1,1]$. We obtain the following explicit bounds.



\begin{lemma}\label{lem:collision_basic}
 The collision probability $p_{+}(\rho)$ is a decreasing function and satisfies:
 \begin{enumerate}
 \item For $|\rho|\leq 1-\delta$, $\frac{\sqrt{2}(1-\zeta)\delta^{2}}{148\sqrt{\pi}} e^{-\frac{1-\rho}{1+\rho}\frac{t^{2}}{2}}\leq p_{+}(\rho) \leq \frac{2}{\sqrt{\pi}\sqrt{\delta}} e^{-\frac{1-\rho}{1+\rho}\frac{t^{2}}{2}}$.
 \item For $1-\delta < \rho \leq 1$, $p_{+}(\rho)\geq \frac{1-\zeta}{2\sqrt{2\pi}(1+\sqrt{2})} e^{-\frac{\delta}{2-\delta} \frac{t^{2}}{2}}$.
 \item For $-1\leq \rho \leq -1+\delta $, $p_{+}(\rho) \leq \frac{2}{\sqrt{\pi}\sqrt{\delta}} e^{-\frac{2-\delta}{\delta}\frac{t^{2}}{2}}$.
\begin{equation}
\nonumber
 \end{equation}
 \end{enumerate}
\end{lemma}

\subsection{Distance Sensitive Hashing on the Sphere}
Given real number $t,\gamma>0$, we define the following hash family $\mathcal{D}_{\gamma}(t,\zeta)$ by sampling a $(h_{+},g_{+})\sim \mathcal{D}_{+}(t,\zeta)$ and $(h_{-},g_{-})\sim \mathcal{D}_{-}(\gamma t, \zeta)$. We create the hash functions by $h_{\gamma}(x) :=(h_{+}(x), h_{-}(x))$ and $g_{\gamma}(x):=(g_{+}(x),g_{-}(x))$ and write $(h_{\gamma}, g_{\gamma})\sim \mathcal{D}_{\gamma}(t,\zeta)$. Define the collision probability $p_{\gamma,t}(\rho):=\P_{(h,g)\sim \mathcal{D}_{\gamma}(t,\zeta)}[h_{\gamma}(x)=g_{\gamma}(y)]$.
\begin{corollary}\label{cor:sensitive_bounds}
 Given constants $\gamma,t>0$ and $\zeta \in (0,\frac{1}{2})$ define $t_{\gamma}=t\max\{\gamma,1\}$ a pair of hash functions $(h_{\gamma},g_{\gamma})\sim \mathcal{D}_{\gamma}(t, \zeta)$ can be evaluated using space and time $O(dt_{\gamma}\log(\frac{1}{\zeta})e^{ t_{\gamma}^{2}/2})$. Furthermore, let $C_{1}(\delta):= \left(\frac{148\sqrt{\pi}}{\sqrt{2}(1-\zeta)\delta^{2}}\right)^{2}$ depending only on $\zeta, \delta$ such that:
\begin{align}
\frac{1}{C_{1}} e^{-\left(\frac{1-\rho}{1+\rho}+\gamma^{2}\frac{1+\rho}{1-\rho}\right)\frac{t^{2}}{2}}\leq p_{\gamma,t}(\rho)&\leq C_{1} e^{-\left(\frac{1-\rho}{1+\rho}+\gamma^{2}\frac{1+\rho}{1-\rho}\right)\frac{t^{2}}{2}},  \ &&\mathrm{for} \ |\rho|\leq 1-\delta\label{eq:tight_sensitive}\\
p_{\gamma,t}(\rho) &\leq  \sqrt{C_{1}(\delta)} e^{-\frac{2-\delta}{\delta}\frac{t_{\gamma}^{2}}{2}}, &&\mathrm{for}   |\rho|>1-\delta\label{eq:tail_sensitive}
\end{align}
\end{corollary}





==> kde.tex <==
\section{Reduction from Euclidean Space to Unit Sphere}
\[
w(x,y)= p_{0}(\|x\|) e^{f(\langle x, y \rangle)-\psi(y)}
\]
The idea behind reducing the problem from a subset of the Euclidean space to the unit Sphere is to partition the dataset $P=\{P_{1},\ldots, P_{K}\}$ into $K$ parts such that within each part the norms differ only by a small multiplicative constant and then pretend as if all the points within each part have the same norms. Given $0<\gamma\leq 1$ a dataset $P$ and any query $x$, define
\begin{align}
r_{0}&=r_{0}(P)=\min\{\|y\|: y\in P, y\neq 0\}\\
R&=R(P,x)=\sup\left\{\|y_{1}-y_{2}\|\bigr|y_{1},y_{2}\in P\cup \{x\}\right\}\\
K &:=K(R/r_{0},\gamma)=\lceil \log(R/r_{0}) / \log(1+\gamma) \rceil
\end{align}
Further for $i\in \mathbb{Z}$ define $S_{i}=[(1+\gamma)^{i-1}r_{0}, (1+\gamma)^{i}r_{0})$ and the corresponding sets:
\begin{equation}
P_{i}:=\{y\in P\bigr|\|y\|\in S_{i}\}, \ i \in [K]
\end{equation}
For any point $x\in \R^{d}$ define $i(x):=\arg\min_{i\in \mathbb{Z}}\{\|x\|\in S_{i}\}$, and its norm-truncated version:
\begin{equation}
\tilde{x}:=\tilde{x}(\gamma) = \frac{x}{\|x\|} (1+\gamma)^{i(x)-1}r_{0} 
\end{equation}
The main lemma we have to prove is the following:
\begin{lemma} Let  where $p_{0}$ is $(L,\delta, S_{i})$-Lipschitz for all $i\in K$ and $f$ is Lipschitz, and define $\tilde{w}(x,y) =p_{0}(\|\tilde{x}\|) \exp\left\{f(\langle \tilde{x},\tilde{y})-\psi(y)\right\}$. Then, $|w(x,y)-\tilde{w}(x,y)| \leq C w(x,y)$.
\end{lemma}
\begin{proof}
Using the definition of $S_{i}$ and the mapping $\tilde{x}$, 
\begin{align}
\qquad\left|\log\left(\frac{p_{0}(\|\tilde{x}\|)}{p_{0}(\|x\|)}\right)\right|  &\leq L\bigl|\log\left(\frac{\|\tilde{x}\|}{\|x\|}\right)\bigr| + \delta\\
&\leq L \gamma  +\delta \\
\Rightarrow \max\left\{ \frac{p_{0}(\|\tilde{x}\|)}{p_{0}(\|x\|)}, \frac{p_{0}(\|x\|)}{p_{0}(\|\tilde{x}\|)}\right\} &\leq e^{L\gamma+\delta}\\
\Rightarrow    e^{-(L\gamma+\delta)}   p_{0}(\|x\|) \leq  p_{0}(\|\tilde{x}\|) \leq e^{L\gamma+\delta} p_{0}(\|x\|)
\end{align}

\end{proof}
Given a hashing based estimator with

$w(x,y)$ we are going to show $w(\tilde{x},\tilde{y})$ is close 
We are going to use this fact and exploit smoothness of the weight function with respect to the norms to argue that the sampling probabilities $p_{*}(x)$ induced by assuming that within each part $P_{i}$ all the norms are constant are very close to the probabilities that 


The notion of smoothness we require is a relaxation of the usual definition of Lipschitz functions.
\begin{definition}
A function $f:\R_{+}\to \R_{+}$ is called $(L,\epsilon, S)$-Lipschitz with respect to a metric $d:\R_{+}\times \R_{+}\to \R_{+}$ if for all $x,y\in S\subseteq \R_{+}$, $d(f(x), f(y)) \leq L \cdot d(x,y) + \epsilon$.
\end{definition}

Given $0<\gamma\leq 1$ define the sets 
The idea
\begin{theorem}
Let $p_{0}:\R_{+}\to \R_{+}$ be a function of $\|x\|$ that is $(L,\epsilon)$-Lipschitz with respect to the Hilbert metric $d_{H}(x,y)=\log(x,y)$. Then given an estimator 
\end{theorem}

 but instead of using the metric $|\cdot|$ we are going to use the Hilbert metric on $\R_{+}$ given $d_{H}(x,y)=\log(x/y)$.
Consider the function: $w(x,y) = \|y\|^{t}\exp\left\{\phi(\|y\|) - A(x) + f(\langle x, y\rangle)\right\}$. Let $L_{*}=\max\{L(\phi), L(f)\}$ and for a given $\delta>0$ set $\gamma= \min\left\{1,\frac{\delta}{L(\phi)R}, \frac{\delta}{3L(f)R^{2}}\right\}$ where $R=\sup_{y\in P\cup \{x\}}\{\|y\|\}$. And let $r_{0}=\min\{y\in P\setminus\{0\}\}\{\|y\|\}$. Set $K=\lceil\frac{\log(\frac{R}{r_{0}})}{\log(1+\gamma)}\rceil = O\left(\frac{\log(R/r_{0}) L_{*}R}{\delta}\right)$. For $i=1,\ldots, K$  let $S_{i}=\{y\in P: (1+\gamma)^{i-1}r_{0} \leq  \|y\|< (1+\epsilon)^{i}\}r_{0}$. Define the mapping $\tilde{x} = \frac{x}{\|x\|}(1+\gamma)^{i(x)-1}r_{0}$ where $i(x) = \arg \min_{i\in [K]}\{x\in S_{i}\}$.
\begin{proposition}For all $y_{1},y_{2}\in S_{i}$, $x_{1},x_{2}\in S_{j}$ we have:
\begin{eqnarray}
\bigl|\|y_{1}\|^{t}-\|y_{2}\|^{t}\bigr| &\leq& \gamma\max\{\|y_{1}\|^{t},\|y_{2}\|^{t}\} \left\{\begin{matrix}
1, & |t|\leq 1\\
2|t|, & |t|>1, \gamma  \leq \frac{1}{2(|t|-1)}
\end{matrix} \right.\\
\biggl|\|y_{1}\|\|x_{1}\| - \|y_{2}\|\|x_{2}\|\biggr| &\leq& 3 R^{2}\gamma
\end{eqnarray} 
\end{proposition}
\begin{proof}
Without loss of generality we assume $\|x_{1}\|\geq \|x_{2}\|$ and $\|y_{1}\|\geq \|y_{2}\|$. We have for $z\in \{x,y\}$:
\begin{eqnarray}
\|z_{1}\|^{t} -\|z_{2}\|^{t} \leq (1+\gamma)^{i(z_{1})}r_{0} - (1+\gamma)^{i(z_{2})-1}r_{0} \leq (1+\gamma)^{i(z_{1})-1}r_{0}\gamma\leq R\gamma
\end{eqnarray}
For the second part:
\begin{align}
\|y_{1}\|\|x_{1}\|-\|y_{2}\|\|x_{2}\| &\leq (1+\gamma)^{i(y_{1})+i(x_{1})}r_{0}^{2} - (1+\gamma)^{i(y_{2})+i(x_{2})-2}r_{0}^{2}\\
&\leq (1+\gamma)^{i(y_{1})+i(x_{1})-2}r_{0}^{2}\left((1+\gamma)^{2}-1 \right)\\
&=3R^{2}\gamma
\end{align}
where we used the fact that $\gamma\leq 1$.
\end{proof}
\begin{corollary}
For any lipschitz function $h$ with constant $L(h)$ we have:
\begin{equation}
h(\|\tilde{x}\|)-h(\|x\|) \leq L(h)R \gamma 
\end{equation}
\end{corollary}
And define the modified weight function $\tilde{w}(x,y)= w(\tilde{x},\tilde{y})$. 
\begin{lemma}
\begin{equation}
|\tilde{w}(x,y) - w(x,y)|\leq e^{2\delta} w(x,y)
\end{equation}
\end{lemma}
\begin{proof}
We first obtain a lower bound:
\begin{align}
\tilde{w}(x,y) = \exp\left\{\phi(\|\tilde{y}\|)-A(x)+f(\langle \tilde{x}, \tilde{y}\rangle)\right\}
\end{align}
We have that:
\begin{align}
 \phi(\tilde{y}) &\geq \phi(y)-L(\phi)(\|y\|-\|\tilde{y}\|) \geq \phi(y)- L(\phi)R\gamma\\
\phi(\tilde{y}) & \leq \phi(y) + L(\phi)(\|y\|-\|\tilde{y}\|) \leq \phi(y) + L(\phi)R\gamma
\end{align}
Similarly we have
\begin{align}
f(\langle \tilde{x}, \tilde{y}\rangle)&\geq f(\langle x, y\rangle) - L(f) (\|x\|\|y\|-\|\tilde{x}\|\|\tilde{y}\|)|\langle \hat{x},\hat{y}\rangle|\geq f(\langle x, y\rangle) - 3L(f)R^{2}\gamma\\ f(\langle \tilde{x}, \tilde{y}\rangle)&\leq f(\langle x, y\rangle) + L(f) (\|x\|\|y\|-\|\tilde{x}\|\|\tilde{y}\|)|\langle \hat{x},\hat{y}\rangle| \leq f(\langle x, y\rangle) + 3L(f)R^{2}\gamma
\end{align}
Putting these two together and using the definition of $\gamma$ we get the required statement
\end{proof}
 
In this section we show that if one has an algorithm to solve the problem $PFE_{P}(q)$ on the unit sphere then, by increasing the query time and space by a factor

\[
e^{-\|x-y\|^{2}} = e^{-\|x\|^{2}} \cdot e^{-\|y\|^{2}} \cdot e^{+2\|x\|\|y\|\langle\hat{x},\hat{y}\rangle}
\]
Let $R=\sup\limits_{x\in P\cup \{q\}}\{\|x\|\}$, and let $S_{i}=\{x: (1+\epsilon)^{i-1} < \|x\|\leq (1+\epsilon)^{i}\}$ with $\epsilon = 1/(2R)^{2}$. Then, 

Let $x\in S_{i}$ then
\[
1 \leq e^{-\|\tilde{x}\|^{2}+\|x\|^{2}} = e^{(\|x\|-\tilde{x}\|)(\|x\|+\|\tilde{x}\|)} \leq e^{[(1+\epsilon)^{i}-(1+\epsilon)^{i-1}]2(1+\epsilon)^{i}} \leq e^{2(1+\epsilon)^{2i}\epsilon} = \sqrt{e}
\]

Assuming $\langle \hat{x},\hat{y}\rangle \geq 0$:
\[
e^{-\epsilon 2R^{2}(2+\epsilon)}\leq e^{2[(1+\epsilon)^{i+j-2}-(1+\epsilon)^{i+j}]}\leq e^{2\langle \hat{x},\hat{y}\rangle (\|\tilde{x}\|\|\tilde{y}\|-\|x\|\|y\|)}\leq 1
\]
\begin{align}
|k(x,y)-k(\tilde{x},\tilde{y})| &= \left| e^{-\|x-y\|^{2}} - e^{-\|\tilde{x}-\tilde{y}\|^{2}}\right|\\
& \left|1- e^{-(\|\tilde{x}\|-\|x\|)(\|\tilde{x}\|+\|x\|)}e^{-(\|\tilde{y}\|-\|y\|)(\|\tilde{y}\|+\|y\|)}e^{2\langle\hat{x},\hat{y}\rangle(\|\tilde{x}\|\tilde{y}\|-\|x\|\|y\|)}\right|\\
&\leq e^{\frac{25}{16}}\cdot  k(x,y)
\end{align}
where $\frac{25}{16}$ can't be made arbitrarily close $0$. Therefore, any importance sampling scheme for $k(x,y)$ will also work for $\tilde{k}(x,y)$. Without loss of generality we may assume that $\|x\|=\|y\|=1$ for all points. In the case of the Partition function estimation problem we need to pick $\epsilon= \frac{1}{2\beta R^{2}}$. Therefore, the number of separate data-structures required are:
\[
\left(\frac{\log (2\beta R^{2})}{\log(1+\frac{1}{2\beta R^{2}})}\right)^{2} = O(\log^{2} (\beta R^{2})\beta^{2} R^{4})
\]
\subsection{Lipschitz- functions}


\begin{align}
|f(c_{1} r) - f(c_{2}r)| \leq L |r||c_{1}-c_{2}| \leq \epsilon
\end{align}



==> logconvex.tex <==
\section{Log-convex Approximation}
\begin{itemize}
\item Local Concave approximation
\item Local Linear Approximation
\item Log-convex approximation
\end{itemize}
